Explaining Drift using Shapley Values

Machine learning models often deteriorate in their performance when they are used to predict the outcomes over data on which they were not trained. These scenarios can often arise in real world when the distribution of data changes gradually or abruptly due to major events like a pandemic. There have been many attempts in machine learning research to come up with techniques that are resilient to such Concept drifts. However, there is no principled framework to identify the drivers behind the drift in model performance. In this paper, we propose a novel framework - DBShap that uses Shapley values to identify the main contributors of the drift and quantify their respective contributions. The proposed framework not only quantifies the importance of individual features in driving the drift but also includes the change in the underlying relation between the input and output as a possible driver. The explanation provided by DBShap can be used to understand the root cause behind the drift and use it to make the model resilient to the drift.

==> introduction.tex <==
% !TEX root = paper.tex
\section{Introduction}
In Machine learning we model a certain quantity of interest as a function of observed variables. This allow us to predict the values of the dependent variables when the values of the independent variables are observed. With the advent of sophisticated models, the function used to represent the variable of interest has also become sophisticated. These sophisticated models like Neural Networks, boosted ensembles etc while being able to accurately map the variables, tend to be non-interpretable. It would require a separate set of tools to interpret the predictions made by these {\em black box} models and identify the features that were responsible for the model to output a particular prediction. In recent years, there has been a lot of development in the area of explainability with a number of explainability methods being proposed. Out of these, the idea of using Shapley values to measure the importances of features has been the most popular. Shapley values have been used to provide a measure of feature importance by fairly assigning the predicted value amongst the features of the model. Hence, given a set of features along with their values, by computing the Shapley values(or its approximation \cite{}), we can assign quantitative values corresponding to the importances of the individual features. The importances are assigned for a particular instance and for a particular set of values taken by the features. The importances of features would change for a different set of values for the features. Feature importances are always measured as a comparison with a baseline - if the value of the function changes from $f(x_{baseline})$ to $f(x_{target})$ for a corresponding change in values from $x_{baseline}$ to $x_{target}$, which among the features of $x$ contributed to the change in $f$ and by how much. In this paper, {\em we extend this to cases when the we want to understand the changes in distribution of the independent variables and how it impacts the distribution of the dependent variable}.

In many applications, we are interested in understanding the effect of distributional change in input affecting the output prediction of a model. For instance, in case of a credit risk model, we observe a change in the distribution of risk score across the population after a recession o. We would then like to understand the reason behind this shift. Specifically, we would like to understand if there are one or more inputs whose distribution had changed leading to the change in the risk score. We often call this change as a {\em data drift}. In another example, we find that a model predicts a certain geographical area to have a higher risk of diabetes compared to another area. In this case, we would like to understand the contributing factor that leads to this change in the distribution. It is important to note that in both these examples our aim is to identify the important features based on how the change in its distribution affects the distribution of the score, unlike the conventional feature importance where the difference in values of features is tracked. In this paper, we develop a framework to address this problem and provide an algorithm to attribute importances to features of black box machine learning models.


